Implementation of airborne ML models with semantics preservation

Machine Learning (ML) may offer new capabilities in airborne systems. However, as any piece of airborne systems, ML-based systems will be required to guarantee their safe operation. Thus, their development will have to be demonstrated to be compliant with the adequate guidance. So far, the European Union Aviation Safety Agency (EASA) has published a concept paper and an EUROCAE/SAE group is preparing ED-324. Both approaches delineate high-level objectives to confirm the ML model achieves its intended function and maintains training performance in the target environment. The paper aims to clarify the difference between an ML model and its corresponding unambiguous description, referred to as the Machine Learning Model Description (MLMD). It then refines the essential notion of semantics preservation to ensure the accurate replication of the model. We apply our contributions to several industrial use cases to build and compare several target models.

==> 08_verification.tex <==
%!TeX root=main.tex
\section{Verification method}
\subsection{Validation of the model properties including margin for~\implmdl prediction errors}
Let us set the required $\varepsilon_{max}$.
We then compute the properties metrics bounds for the use case based on $f_1(x)$,  $f(x)$ and $\varepsilon_{max}$.
These bounds shall be validated by the model designer as the last activity of the first V-cycle development process.

\begin{figure}[hbt]
	\tiny
	\centering
	\resizebox{0.3\textwidth}{!}{%
	\begin{tikzpicture}
	\node [rectangle, minimum height = .5cm,draw] (valset) at (0,0.7){\begin{tabular}{l}Validation/Test\\set input\end{tabular}};
	\node [rectangle, minimum height = .5cm,draw] (gt) at (0,0){Ground truth};
	\node [rectangle, minimum height = .5cm,draw] (tfm) at (1.5,0.7){\trainmdl};
	\node [rectangle, minimum height = .5cm,draw] (pred) at (3,0.7){\trainmdl predictions};
	\node [rectangle, minimum height = .5cm,draw] (eps) at (5.5,0.7){$\varepsilon_{max}$};
	\node [rectangle, minimum height = .5cm,draw] (val) at (4,0){\begin{tabular}{l}Metrics\\validation\end{tabular}};

	\draw [-Latex] (valset) --   (tfm);
	\draw [-Latex] (tfm) --   (pred);
	\draw [-Latex] (gt) --   (val);
	\draw [-Latex] (eps) |-   (val);
	\draw [-Latex] (pred) -|   (val);
	\end{tikzpicture}
	}%
	\caption{Metrics validation\label{fig:validation}}
\end{figure}

\subsection{Cross-verification of the \trainmdl and the \onnx MLMD}
The verification of the \emph{SL2} is performed by review of the model DAG structure. 
The review is based on trace data included in MLMD linked to the \trainmdl.
The MLMD and \trainmdl have the same SL2 semantics, if the symbolic expression of each output tensor element are identicals.
This verification might be automated by a symbolic solver, but is not in the scope of this paper.
Ex:
\trainmdl: $f(x) = xW+b$ identical to MLMD : $f(x) = b+(W^Tx)^T$

\subsection{Replication metrics verification}
Using the~\implmdl, we compute the predictions $\hat f_2(x_i)$,
and the $\varepsilon_i = \hat f_2(x_i) - \hat f_1(x_i)$ using the $\hat f_1(x_i)$ provided by the model designer.

Then we assert that $|\varepsilon_i| \leq \varepsilon_{max} \forall i \in [1,n]$. 
The validated ML properties are preserved if the $\varepsilon$ criteria holds. If the criteria does not hold, we cannot conclude. 
Note that for this activity, any dataset might be used, i.e. the test-set, the training-set or a synthetically (Latin-Hypercube) sampled dataset.
\begin{figure}[hbt]
	\tiny
	\centering
	\resizebox{0.3\textwidth}{!}{%
	\begin{tikzpicture}
	\node [rectangle, minimum height = .5cm,draw] (input) at (-1,0){\begin{tabular}{l}Replication set\\input\end{tabular}};
	\node [rectangle, minimum height = .5cm,draw] (eps) at (7,0.5){$\varepsilon_{max}$};
	\node [rectangle, minimum height = .5cm,draw] (tar) at (1,-0.5){\implmdl};
	\node [rectangle, minimum height = .5cm,draw] (tfm) at (1,0.5){\trainmdl};
	\node [rectangle, minimum height = .5cm,draw] (tarpred) at (3,-0.5){\begin{tabular}{l}\implmdl\\predictions\end{tabular}};
	\node [rectangle, minimum height = .5cm,draw] (tfmpred) at (3,0.5){\trainmdl predictions};
	\node [rectangle, minimum height = .5cm,draw] (sts) at (5,0){\begin{tabular}{l}Replication\\status\end{tabular}};
       
	\draw [-Latex] (input) |-   (tar);
	\draw [-Latex] (input) |-   (tfm);
	\draw [-Latex] (tfm) --   (tfmpred);
	\draw [-Latex] (tar) --   (tarpred);
	\draw [-Latex] (tarpred) -|   (sts);
	\draw [-Latex] (tfmpred) -|   (sts);
	\draw [-Latex] (eps) |-   (sts);
	\end{tikzpicture}
	}%
	\caption{Replication verification\label{fig:verification}}
\end{figure}


